Drillboards: Adaptive Visualization Dashboards for Dynamic Personalization of Visualization Experiences

We present drillboards, a technique for adaptive visualization dashboards consisting of a hierarchy of coordinated charts that the user can drill down to reach a desired level of detail depending on their expertise, interest, and desired effort. This functionality allows different users to personalize the same dashboard to their specific needs and expertise. The technique is based on a formal vocabulary of chart representations and rules for merging multiple charts of different types and data into single composite representations. The drillboard hierarchy is created by iteratively applying these rules starting from a baseline dashboard, with each consecutive operation yielding a new dashboard with fewer charts and progressively more abstract and simplified views. We also present an authoring tool for building drillboards and show how experts users can use to build up and deliver personalized experiences to a wide audience. Our evaluation asked three domain experts to author drillboards for their own datasets, which we then showed to casual end-users with favorable outcomes.

==> content/abstract.tex <==
% --------------------------------------------------------------------------------
% Abstract
% --------------------------------------------------------------------------------
\begin{abstract}
    We present \textit{drillboards}, a technique for adaptive visualization dashboards consisting of a hierarchy of coordinated charts that the user can drill down to reach a desired level of detail depending on their expertise, interest, and desired effort.
    This functionality allows different users to personalize the same dashboard to their specific needs and wants.
    The technique is based on a formal vocabulary of chart representations and rules for merging multiple charts of different types and data into single composite representations.
    The drillboard hierarchy is created by iteratively applying these rules starting from a baseline dashboard, with each consecutive operation yielding a new dashboard with fewer charts and progressively more abstract and simplified views.
    We also present an authoring tool for building drillboards and show how it can be applied to an agricultural dataset with hundreds of expert users.
    %% Evaluation?
\end{abstract}


==> content/scraps.tex <==

% The goal of developing an interface is to provide different levels of summarization based on different levels of knowledge, and thereby provide an effective delivery of information that matches the readers' details of knowledge.
% For this, we devise five design goals in building the system. 

% \begin{itemize}[noitemsep, topsep=0.2em, leftmargin=2.5em]

%     \item [\textbf{DG1}] \textbf{Multi-level comprehensible:} The dashboard should satisfy the level of detail from people with different expertise levels.
%     PolyZoom lets users focus on multi zoom levels on a geographic map simultaneously~\cite{Javed2012}.
%     In DrillBoards, different levels of detail are provided upon the user's choice by presenting information from different levels of the tree, under one identical structure. 
%     % This is the goal
%     % Multi-level explainability, and multi-level expandability is different. 
%     \item [\textbf{DG2}] \textbf{Multi-focus drilldown:} Users should be able to explore, or drill down into different levels of details.
%     Users can have multiple points of focus they can drill down. 
%     %~\cite{Elmqvist2008d}.
%     % This is the goal
%     \item [\textbf{DG3}] \textbf{Intuitive:} Visual representations, designs and metaphors used in the interface must be easy and intuitive so that users can easily understand how the tool works. 
%     % Easy to use (good metaphors)
%     \item [\textbf{DG4}] \textbf{Explainable:} At the same time, the dashboard should also inform users about how the hierarchy is formed.   
%     \item [\textbf{DG5}] \textbf{Responsive:} As this dashboard deals with large scale information, users might want to change the resolution and see the drillboards in a larger view, or smaller views. 
%     The system should be able to keep consistency~\cite{kim22cicero} under different window sizes, so that users do not feel confused.
%     % Provide explanation for good guessing
%     %how can you accommodate large-scale data? (scalable)
%     %how will you explain so that the user understands the operation? (explainable)
    
% \end{itemize}

%We propose DrillVis, a monitoring tool for tabular datasets, which effectively summarizes charts through an aggregation of charts that efficiently presents different [gotta write this after I read more papers]

